Spike-and-Slab LASSO Generalized Additive Models and Scalable Algorithms for High-Dimensional Data Analysis

There are proposals that extend the classical generalized additive models (GAMs) to accommodate high-dimensional data ($p>>n$) using group sparse regularization. However, the sparse regularization may induce excess shrinkage when estimating smooth functions, damaging predictive performance. Moreover, most of these GAMs consider an "all-in-all-out" approach for functional selection, rendering them difficult to answer if nonlinear effects are necessary. While some Bayesian models can address these shortcomings, using Markov chain Monte Carlo algorithms for model fitting creates a new challenge, scalability. Hence, we propose Bayesian hierarchical generalized additive models as a solution: we consider the smoothing penalty for proper shrinkage of curve interpolation via reparameterization. A novel two-part spike-and-slab LASSO prior for smooth functions is developed to address the sparsity of signals while providing extra flexibility to select the linear or nonlinear components of smooth functions. A scalable and deterministic algorithm, EM-Coordinate Descent, is implemented in an open-source R package BHAM. Simulation studies and metabolomics data analyses demonstrate improved predictive and computational performance against state-of-the-art models. Functional selection performance suggests trade-offs exist regarding the effect hierarchy assumption.

==> Tabs/sim_binom_var_slct_tab.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{cccccccc}
  \hline
P & Metric & LASSO & COSSO & Adaptive COSSO & BHAM & SB-GAM & spikeSlabGAM \\ 
  \hline
  4 & Precision & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\ 
   10 & Precision & 0.58 & 0.71 & 0.69 & 0.93 & 0.88 & 0.89 \\ 
   50 & Precision & 0.38 & 0.60 & 0.59 & 0.77 & 0.80 & 0.52 \\ 
  100 & Precision & 0.35 & 0.62 & 0.65 & 0.82 & 0.77 & 0.42 \\ 
  200 & Precision & 0.29 & 0.65 & 0.57 & 0.21 & 0.74 & 0.36 \\ 
   \hline
  4 & Recall & 0.54 & 0.61 & 0.54 & 0.38 & 0.97 & 0.55 \\ 
   10 & Recall & 0.46 & 0.50 & 0.54 & 0.38 & 0.97 & 0.54 \\ 
   50 & Recall & 0.34 & 0.30 & 0.30 & 0.32 & 0.90 & 0.55 \\ 
  100 & Recall & 0.27 & 0.30 & 0.25 & 0.27 & 0.92 & 0.54 \\ 
  200 & Recall & 0.27 & 0.25 & 0.29 & 0.56 & 0.92 & 0.53 \\ 
   \hline
 10 & MCC & 0.18 & 0.35 & 0.36 & 0.47 & 0.86 & 0.55 \\ 
   50 & MCC & 0.25 & 0.34 & 0.36 & 0.45 & 0.83 & 0.47 \\ 
  100 & MCC & 0.24 & 0.37 & 0.37 & 0.45 & 0.82 & 0.43 \\ 
  200 & MCC & 0.23 & 0.36 & 0.36 & 0.23 & 0.81 & 0.40 \\ 
   \hline
\end{tabular}
\caption{The variable selection performance of binomial simulations,
                         measured by positive predictive value (precision), true positive rate (recall),
                         and Matthews correlation coefficient (MCC), for the high-dimensional methods 
                         averaged over 50 iterations. The models of comparison include the proposed Bayesian
                         hierarchical additive model (BHAM), linear LASSO model (LASSO), component selection and
                         smoothing operator (COSSO), adaptive COSSO, sparse Bayesian generalized additive model (SB-GAM),
                         and spikeSlabGAM model. MCC is ill-defined when $p=4$ simulation (no true negative), and hence omitted for all methods.} 
\label{tab:sim_binom_var_select}
\end{table}


==> Tabs/sim_lnr_binom_tab.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{cccccccc}
  \hline
P & mgcv & LASSO & COSSO & Adaptive COSSO & BHAM & SB-GAM & spikeSlabGAM \\ 
  \hline
  4 & 0.79 (0.01) & 0.79 (0.01) & 0.76 (0.04) & 0.75 (0.04) & 0.78 (0.01) & 0.76 (0.01) & 0.79 (0.01) \\ 
   10 & 0.77 (0.01) & 0.79 (0.01) & 0.78 (0.01) & 0.78 (0.01) & 0.78 (0.01) & 0.75 (0.01) & 0.79 (0.01) \\ 
   50 & 0.62 (0.01) & 0.78 (0.01) & 0.75 (0.03) & 0.73 (0.04) & 0.74 (0.07) & 0.75 (0.02) & 0.77 (0.01) \\ 
  100 & - & 0.78 (0.01) & 0.73 (0.04) & 0.69 (0.05) & 0.73 (0.07) & 0.74 (0.02) & 0.76 (0.02) \\ 
  200 & - & 0.78 (0.01) & 0.71 (0.05) & 0.67 (0.05) & 0.73 (0.06) & 0.73 (0.03) & 0.72 (0.03) \\ 
   \hline
\end{tabular}
\caption{The average and standard deviation of the out-of-sample area under the curve measures
    for binomial outcomes over 50 iterations. The models of comparison include the proposed
    Bayesian hierarchical additive model (BHAM), linear LASSO model (LASSO), component
    selection and smoothing operator (COSSO), adaptive COSSO, mgcv, sparse Bayesian
    generalized additive model (SB-GAM), and spikeSlabGAM model. mgcv doesn't provide
    estimation when number of parameters exceeds sample size i.e. p = 100, 200.} 
\label{tab:lnr_bin_auc}
\end{table}


==> Tabs/sim_lnr_binom_var_slct_tab.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{cccccccc}
  \hline
P & Metric & LASSO & COSSO & Adaptive COSSO & BHAM & SB-GAM & spikeSlabGAM \\ 
  \hline
  4 & Precision & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\ 
   10 & Precision & 0.61 & 0.97 & 0.98 & 0.55 & 0.74 & 0.91 \\ 
   50 & Precision & 0.35 & 0.59 & 0.68 & 0.26 & 0.59 & 0.61 \\ 
  100 & Precision & 0.28 & 0.47 & 0.51 & 0.30 & 0.46 & 0.57 \\ 
  200 & Precision & 0.26 & 0.44 & 0.42 & 0.38 & 0.41 & 0.38 \\ 
   \hline
  4 & Recall & 1.00 & 0.85 & 0.78 & 1.00 & 1.00 & 1.00 \\ 
   10 & Recall & 1.00 & 0.96 & 0.97 & 0.99 & 1.00 & 1.00 \\ 
   50 & Recall & 1.00 & 0.88 & 0.74 & 0.92 & 1.00 & 1.00 \\ 
  100 & Recall & 1.00 & 0.78 & 0.56 & 0.89 & 1.00 & 0.99 \\ 
  200 & Recall & 1.00 & 0.67 & 0.48 & 0.89 & 0.99 & 0.98 \\ 
   \hline
 10 & MCC & 0.58 & 0.95 & 0.96 & 0.49 & 0.72 & 0.91 \\ 
   50 & MCC & 0.52 & 0.66 & 0.65 & 0.37 & 0.73 & 0.74 \\ 
  100 & MCC & 0.49 & 0.55 & 0.47 & 0.43 & 0.65 & 0.72 \\ 
  200 & MCC & 0.49 & 0.49 & 0.39 & 0.47 & 0.62 & 0.58 \\ 
   \hline
\end{tabular}
\caption{The variable selection performance of linear binomial simulations,
                         measured by positive predictive value (precision), true positive rate (recall),
                         and Matthews correlation coefficient (MCC), for the high-dimensional methods
                         averaged over 50 iterations. The models of comparison include the proposed Bayesian
                         hierarchical additive model (BHAM), linear LASSO model (LASSO), component selection
                         and smoothing operator (COSSO), adaptive COSSO, sparse Bayesian generalized
                         additive model (SB-GAM), and spikeSlabGAM model. MCC is ill-defined when $p=4$
                         simulation (no true negative), and hence omitted for all methods.} 
\label{tab:sim_lnr_binom_var_select}
\end{table}


==> Tabs/sim_lnr_gaus_tab.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{cccccccc}
  \hline
P & mgcv & LASSO & COSSO & Adaptive COSSO & BHAM & SB-GAM & spikeSlabGAM \\ 
  \hline
  4 & 0.38 (0.01) & 0.39 (0.01) & 0.31 (0.08) & 0.29 (0.11) & 0.38 (0.01) & 0.35 (0.01) & 0.39 (0.01) \\ 
   10 & 0.36 (0.02) & 0.38 (0.01) & 0.35 (0.03) & 0.34 (0.04) & 0.39 (0.01) & 0.33 (0.02) & 0.39 (0.01) \\ 
   50 & 0.09 (0.09) & 0.37 (0.01) & 0.30 (0.06) & 0.30 (0.36) & 0.38 (0.01) & 0.32 (0.03) & 0.37 (0.01) \\ 
  100 & - & 0.37 (0.01) & 0.28 (0.07) & 0.34 (0.04) & 0.38 (0.01) & 0.29 (0.07) & 0.35 (0.01) \\ 
  200 & - & 0.36 (0.01) & 0.26 (0.08) & 0.31 (0.06) & 0.38 (0.03) & 0.28 (0.06) & 0.33 (0.02) \\ 
   \hline
\end{tabular}
\caption{The average and standard deviation of the out-of-sample $R^2$ measure for
    Gaussian outcomes over 50 iterations. The models of comparison include the proposed
    Bayesian hierarchical additive model (BHAM), linear LASSO model (LASSO), component
    selection and smoothing operator (COSSO), adaptive COSSO, mgcv, sparse Bayesian
    generalized additive model (SB-GAM), and spikeSlabGAM model. mgcv doesn't provide estimation
    when number of parameters exceeds sample size i.e. p = 100, 200.} 
\label{tab:lnr_gaus}
\end{table}


==> Tabs/sim_lnr_gaus_var_slct_tab.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{cccccccc}
  \hline
P & Metric & LASSO & COSSO & Adaptive COSSO & BHAM & SB-GAM & spikeSlabGAM \\ 
  \hline
  4 & Precision & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\ 
   10 & Precision & 0.59 & 0.97 & 0.97 & 0.90 & 0.56 & 0.99 \\ 
   50 & Precision & 0.43 & 0.74 & 0.84 & 0.89 & 0.39 & 0.99 \\ 
  100 & Precision & 0.34 & 0.53 & 0.72 & 0.91 & 0.29 & 0.99 \\ 
  200 & Precision & 0.27 & 0.42 & 0.52 & 0.92 & 0.33 & 0.99 \\ 
   \hline
  4 & Recall & 1.00 & 0.87 & 0.84 & 1.00 & 1.00 & 1.00 \\ 
   10 & Recall & 1.00 & 0.98 & 0.96 & 1.00 & 1.00 & 1.00 \\ 
   50 & Recall & 1.00 & 0.85 & 0.99 & 1.00 & 1.00 & 1.00 \\ 
  100 & Recall & 1.00 & 0.84 & 0.97 & 1.00 & 1.00 & 1.00 \\ 
  200 & Recall & 1.00 & 0.78 & 0.88 & 1.00 & 0.98 & 1.00 \\ 
   \hline
 10 & MCC & 0.59 & 0.96 & 0.94 & 0.91 & 0.54 & 0.99 \\ 
   50 & MCC & 0.59 & 0.76 & 0.90 & 0.92 & 0.57 & 1.00 \\ 
  100 & MCC & 0.54 & 0.61 & 0.81 & 0.94 & 0.48 & 1.00 \\ 
  200 & MCC & 0.49 & 0.52 & 0.64 & 0.95 & 0.52 & 0.99 \\ 
   \hline
\end{tabular}
\caption{The variable selection performance of linear Gaussian
                         simulations, measured by positive predictive value (precision),
                         true positive rate (recall), and Matthews correlation coefficient (MCC),
                         for the high-dimensional methods averaged over 50 iterations.
                         The models of comparison include the proposed Bayesian hierarchical additive model (BHAM),
                         linear LASSO model (LASSO), component selection and smoothing operator (COSSO),
                         adaptive COSSO, sparse Bayesian generalized additive model (SB-GAM), and spikeSlabGAM model.
                         MCC is ill-defined when $p=4$ simulation (no true negative), and hence omitted for all methods.} 
\label{tab:sim_lnr_gaus_var_select}
\end{table}

